Domain-Invariant and Language-Model-Assisted Acoustic Side-Channel Attacks on Keyboards

Acoustic side-channel attacks (ASCA) recover typed text from the sound of keystrokes, using only a commodity microphone and no access to the victim's device. Prior work establishes that such attacks succeed under idealized laboratory conditions - a single keyboard, a fixed microphone, a quiet room, and training and testing on the same device but leaves open the question that matters for security: whether keystroke inference survives the open world of unseen keyboards, diverse users, noisy environments, and compressed transmission channels. The answer developed here is that it does, provided the acoustic model is made explicitly domain-invariant and its noisy predictions are corrected by a language model.

==> frontmatter/cv.tex <==
%--------------------- Curriculum Vitae (Annex I) ---------------------
\chapter*{Curriculum Vitae}
\addcontentsline{toc}{chapter}{Curriculum Vitae}
\markboth{Curriculum Vitae}{}

\noindent\textbf{\large Bikrant Bikram Pratap Maurya}\\[2pt]
Roll No.\ MT24116 \quad$\vert$\quad Email: bikrant24116@iiitd.ac.in\\
Department of Computer Science and Engineering,
Indraprastha Institute of Information Technology Delhi.

\vspace{0.5cm}
\section*{Education}
\begin{itemize}[leftmargin=1.4em,itemsep=3pt]
\item Master of Technology, Computer Science and Engineering (Specialization in Information
Security), Indraprastha Institute of Information Technology Delhi, 2024--2026.
\item \emph{[Bachelor's degree, institution, and year --- to be filled by the candidate.]}
\end{itemize}

\section*{Research Interests}
Acoustic side-channel attacks and security; speech representation learning; domain adaptation
and invariant representation learning; large language models for sequence reconstruction;
applied machine learning for audio.

\section*{Publications}
\begin{itemize}[leftmargin=1.4em,itemsep=3pt]
\item ``DECKER: Domain-invariant Embedding for Cross-Keyboard Extraction and Recognition,''
ACM ASIACCS 2026.
\item ``Impact Analysis of Speech Representation Learning Models for Acoustic Side-Channel
Attack,'' 2026 (arXiv:2606.21210).
\item ``Surviving the Codec: Continuous Sparse Transduction for Acoustic Side-Channel Attacks
over VoIP,'' Interspeech 2026 (under review).
\end{itemize}

\section*{Technical Skills}
Python, PyTorch, and Hugging Face Transformers; digital signal and audio processing (librosa,
torchaudio); self-supervised speech models (Wav2Vec2, WavLM, HuBERT, Whisper); ECAPA-TDNN and
contrastive/adversarial representation learning; large language models and constrained decoding.

\section*{Thesis Summary}
M.Tech.\ thesis on domain-invariant and language-model-assisted acoustic side-channel attacks on
keyboards, introducing the \hear{} dataset and the \decker{} framework, together with
VoIP-channel robustness studies (speech-representation analysis and the \evflow{} continuous
transduction model), under the supervision of Dr.\ Arun Balaji Buduru.

\clearpage


==> frontmatter/titlepage.tex <==
%--------------------- Page 1: Cover Page (Annex I) ---------------------
\begin{titlepage}
\thispagestyle{empty}
\centering
\vspace*{1.2cm}

{\LARGE\bfseries\color{iiitblue}
Domain-Invariant and Language-Model-Assisted\\[0.35cm]
Acoustic Side-Channel Attacks on Keyboards\par}

\vspace{2.2cm}
{\large by\par}
\vspace{0.5cm}
{\Large\bfseries Bikrant Bikram Pratap Maurya\par}

\vspace{2.0cm}
{\large Under the Supervision of\par}
\vspace{0.3cm}
{\large\bfseries Dr.\ Arun Balaji Buduru\par}

\vspace{2.2cm}

\IfFileExists{logo.jpg}{\includegraphics[width=3cm]{logo.jpg}}{%
  \begin{tikzpicture}
  \node[circle,draw=iiitblue,line width=1.2pt,minimum size=2.1cm,
        align=center,text=iiitblue,font=\bfseries] {IIIT\\D};
  \end{tikzpicture}}

\vspace{1.0cm}
{\large\bfseries Indraprastha Institute of Information Technology Delhi\par}
\vspace{0.4cm}
{\large August, 2026\par}

\vfill
\end{titlepage}
\clearpage

